Enhancing Human Evaluation in Machine Translation with Comparative Judgment

Human evaluation is crucial for assessing rapidly evolving language models but is influenced by annotator proficiency and task design. This study explores the integration of comparative judgment into human annotation for machine translation (MT) and evaluates three annotation setups-point-wise Multidimensional Quality Metrics (MQM), side-by-side (SxS) MQM, and its simplified version SxS relative ranking (RR). In MQM, annotators mark error spans with categories and severity levels. SxS MQM extends MQM to pairwise error annotation for two translations of the same input, while SxS RR focuses on selecting the better output without labeling errors. Key findings are: (1) the SxS settings achieve higher inter-annotator agreement than MQM; (2) SxS MQM enhances inter-translation error marking consistency compared to MQM by, on average, 38.5% for explicitly compared MT systems and 19.5% for others; (3) all annotation settings return stable system rankings, with SxS RR offering a more efficient alternative to (SxS) MQM; (4) the SxS settings highlight subtle errors overlooked in MQM without altering absolute system evaluations. To spur further research, we will release the triply annotated datasets comprising 377 ZhEn and 104 EnDe annotation examples.

==> sections/discussion.tex <==
\section{Discussion}

The results of this study elucidate the comparative effectiveness of three annotation settings on human annotators' assessments of machine translation systems. Three key dimensions are explored: system/segment-level rankings, inter/intra-annotator agreement, and annotators' behaviors within the different annotation frameworks.

Concerning the system-level rankings, all three annotation settings provided identical rankings for \ZhEn~with slight divergence on \EnDe. This underscores the robustness of the three annotation settings in that they are reliable in returning stable overall quality assessments. However, such assessment display certain noise at the segment level where the three annotation settings only moderately agree with each other.

Regarding consistency between and within annotators, 
the results reveal that \sxsmqm~slightly improves inter-annotator agreement over MQM but achieves a remarkable increase in inter-translation consistency. Such an improvement highlights the effectiveness of \sxsmqm~in fostering precise and consistent annotations regardless of whether two items are annotated \sxs. This promotes a more standardized annotation process.

Overall, if comprehensive error identification is the priority, MQM is preferable. For consistent and reliable error annotation and robust system rankings, \sxsmqm~is recommended although \sxsmqm~might inadvertently steer annotators toward focusing on differences that more clearly differentiate systems (e.g., accuracy errors), potentially overlooking minor errors (e.g., fluency). Lastly, if one's primary goal is system ranking without detailed error analysis, \sxsqr~offers a comparable performance to more sophisticated methods while requiring only a third of the time.

% \subsection{Suggestions for future human evaluation}

% \yscomment{to be revised}


% Given the results, if comprehensive error identification is the priority, MQM is preferable because \sxsmqm~might inadvertently steer annotators toward focusing on differences that better differentiate systems (e.g., accuracy errors), potentially overlooking minor errors (e.g., fluency). However, \sxsmqm~provides significantly more consistent and reliable error annotation. Lastly, if one's primary goal is system ranking but not detailed error analysis, \sxsqr~offers performance on a par with more sophisticated methods while requiring considerably less time.


==> tables/minor_major_error_perc.tex <==
\begin{table}[htbp]
    % \fontsize{5}{6}\selectfont
    \centering
    % \renewcommand{\arraystretch}{0.8} % Reduce vertical space
    \resizebox{0.95\columnwidth}{!}{%
    \begin{tabular}{@{}rrrrrr@{}}
    \midrule
     & \textbf{Setting} & \textbf{Minor (\%)} & \textbf{Major (\%)} & \textbf{Total count} & \textbf{Avg. Err Len}\\\midrule
    % \multirow{2}{*}{\ZhEn} & MQM & 75.53 & 24.47 & 23469 & 3.37 \\
    %  & \sxsmqm  & 62.43 & 37.57 & 21138 & 2.85\\\midrule
    
    \multirow{2}{*}{\ZhEn} & MQM & 79.44 & 20.56 & 13275 & 3.07 \\
     & \sxsmqm  & 64.19 & 35.81 & 9779 & 2.73  \\\midrule
    
    % \multirow{2}{*}{\EnDe} & MQM & 74.76 & 25.24 & 9977 & 1.96 \\
    %  & \sxsmqm & 75.21 & 24.79 & 9457 & 2.13 \\\midrule
    
    \multirow{2}{*}{\EnDe} & MQM & 74.76 & 25.24 & 9977 &  1.94 \\
     & \sxsmqm & 75.21 & 24.79 & 9457 & 2.05  \\\midrule
     
    \end{tabular}%
    }
    \caption{Percentage and total count of minor and major errors for each language pair and annotation setting. Average error length is measured by the average words per error span, with words split by whitespace.
    }
    \label{tab:error_count_stats}
    % /data/yixiao/human_eval_proj/code_error_distribution/count_error.py
\end{table}

==> tables/system_ranking_orig_w_56225225.tex <==
\begin{table*}[t]
\centering
\begin{minipage}[t]{0.47\textwidth}
    \fontsize{6}{7}\selectfont
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}rrrr@{}}
    \midrule
    \textbf{Setting}   & \textbf{Better System} & \textbf{Worse System} & \textbf{\textit{p} value} \\ \midrule

    \psxsmqm & Lan-BridgeMT (2.13) & GPT4-5shot (2.26)   & 0.121 \\
    \sxsmqm  & Lan-BridgeMT (2.66) & GPT4-5shot (2.81)   & 0.117 \\
    \sxsqr   & Lan-BridgeMT (0.37) & GPT4-5shot (0.44)   & \textbf{0.028} \\\midrule

    \psxsmqm & HW-TSC (3.07)       & ONLINE-A (3.21)     & 0.146 \\
    \sxsmqm  & HW-TSC (3.56)       & ONLINE-A (3.77)     & 0.055 \\
    \sxsqr   & HW-TSC (0.32)       & ONLINE-A (0.50)     & \textbf{0.000} \\\midrule

    \psxsmqm & ONLINE-B (3.35)     & IOL\_Research (3.48) & 0.196 \\
    \sxsmqm  & ONLINE-B (3.68)     & IOL\_Research (4.14) & \textbf{0.001} \\
    \sxsqr   & ONLINE-B (0.32)     & IOL\_Research (0.55) & \textbf{0.000} \\\midrule

    \psxsmqm & ONLINE-W (4.09)     & NLLB\_Greedy (6.73) & \textbf{0.000} \\
    \sxsmqm  & ONLINE-W (4.60)     & NLLB\_Greedy (7.01) & \textbf{0.000} \\
    \sxsqr   & ONLINE-W (0.24)     & NLLB\_Greedy (0.76) & \textbf{0.000} \\\midrule

    \psxsmqm & ONLINE-M (5.04)     & NLLB\_BLEU (6.68)   & \textbf{0.000} \\
    \sxsmqm  & ONLINE-M (5.60)     & NLLB\_BLEU (7.33)   & \textbf{0.000} \\
    \sxsqr   & ONLINE-M (0.26)     & NLLB\_BLEU (0.62)   & \textbf{0.000} \\\midrule
    
    \end{tabular}%
    }
    \caption*{(a) Chinese $\rightarrow$ English} % Label for the left table
\end{minipage}
\hspace{0.03\textwidth} % Add space between the tables
\begin{minipage}[t]{0.47\textwidth}
    \fontsize{6}{7}\selectfont
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}rrrr@{}}
    \midrule
    \textbf{Setting}   & \textbf{Better System} & \textbf{Worse System} & \textbf{\textit{p} value} \\ \midrule

    \psxsmqm & ONLINE-W (3.49) & GPT4-5shot (3.90)  & 0.083 \\
    \sxsmqm  & ONLINE-W (2.72) & GPT4-5shot (3.08)  & 0.095 \\
    \sxsqr   & ONLINE-W (0.33) & GPT4-5shot (0.45)  & 0.058 \\\midrule

    \psxsmqm & ONLINE-A (4.70) & ONLINE-Y (5.13)    & 0.078 \\
    \sxsmqm  & ONLINE-A (3.92) & ONLINE-Y (4.44)    & \textbf{0.018} \\
    \rowcolor{red!8} \sxsqr   & ONLINE-Y (0.38) & ONLINE-A (0.43)    & 0.275 \\\midrule

    \psxsmqm & ONLINE-M (5.83) & ONLINE-G (6.72)    & 0.051 \\
    \sxsmqm  & ONLINE-M (5.45) & ONLINE-G (5.99)    & 0.11  \\
    \sxsqr   & ONLINE-M (0.43) & ONLINE-G (0.44)    & 0.458 \\\midrule

    \psxsmqm & refA (3.18)     & GPT4-5shot (3.90)  & \textbf{0.013} \\
    \rowcolor{red!8} \sxsmqm  & GPT4-5shot (2.86) & refA (3.10)      & 0.270 \\
    \sxsqr   & refA (0.36)     & GPT4-5shot (0.50)  & \textbf{0.036} \\\midrule

    \psxsmqm & Lan-BridgeMT (8.69) & NLLB\_BLEU (10.51) & \textbf{0.003} \\
    \sxsmqm  & Lan-BridgeMT (7.80) & NLLB\_BLEU (10.38) & \textbf{0.000} \\
    \sxsqr   & Lan-BridgeMT (0.22) & NLLB\_BLEU (0.86)  & \textbf{0.000} \\\midrule

    \end{tabular}%
    }
    \caption*{(b) English $\rightarrow$ German} % Label for the left table
\end{minipage}
\caption{Pairwise system rankings and statistical significance of system quality differences for \ZhEn~and \EnDe~under three annotation settings.  The red highlight indicates where an annotation setting yields a different ranking based on scores. Bold \textit{p} values represent statistically significant differences in quality between systems, determined by a random permutation test.}
\label{tab:system_rankings}
\end{table*}
